Autonomous Recharging and Flight Mission Planning for Battery-operated Autonomous Drones

Unmanned aerial vehicles (UAVs), commonly known as drones, are being increasingly deployed throughout the globe as a means to streamline monitoring, inspection, mapping, and logistic routines. When dispatched on autonomous missions, drones require an intelligent decision-making system for trajectory planning and tour optimization. Given the limited capacity of their onboard batteries, a key design challenge is to ensure the underlying algorithms can efficiently optimize the mission objectives along with recharging operations during long-haul flights. With this in view, the present work undertakes a comprehensive study on automated tour management systems for an energy-constrained drone: (1) We construct a machine learning model that estimates the energy expenditure of typical multi-rotor drones while accounting for real-world aspects and extrinsic meteorological factors. (2) Leveraging this model, the joint program of flight mission planning and recharging optimization is formulated as a multi-criteria Asymmetric Traveling Salesman Problem (ATSP), wherein a drone seeks for the time-optimal energy-feasible tour that visits all the target sites and refuels whenever necessary. (3) We devise an efficient approximation algorithm with provable worst-case performance guarantees and implement it in a drone management system, which supports real-time flight path tracking and re-computation in dynamic environments. (4) The effectiveness and practicality of the proposed approach are validated through extensive numerical simulations as well as real-world experiments.

==> authors.tex <==
\vspace*{-15mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/rashid.jpg}}]%
{Rashid Alyassi} received the B.S. degree in Computer Engineering and the M.S. degree in Computer and Information Science both from Khalifa University, UAE, in 2017 and 2020, respectively. Currently, he is a Research Engineer with Khalifa University, UAE. His research interests are centered primarily on Autonomous Vehicles, design and analysis of algorithms, robotics, and Artificial Intelligence.
\end{IEEEbiography}

\vspace*{-15mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/majid.png}}]%
{Majid Khonji} is an assistant professor in the EECS department at Khalifa University, UAE, and a research Affiliate with MIT Computer Science and Artificial Intelligence Laboratory (CSAIL), USA. He received his MSc degree in Security, Cryptology, and Coding of Information Systems from Ensimag, Grenoble Institute of Technology, France, and PhD in Interdisciplinary Engineering from Masdar Institute, UAE, in collaboration with MIT in 2016. Previously, he was a visiting assistant professor with MIT CSAIL, a senior R\&D technologist in Dubai Electricity and Water Authority (DEWA), and an information security researcher in Emirates Advanced Investment Group (EAIG).
\end{IEEEbiography}
\vspace*{-10mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/areg3.jpg}}]%
	{Areg Karapetyan} received the B.S. degree (with honours) in industrial electronics from National Polytechnic University of Armenia in 2010 and in 2015 the M.S. degree in Computing and Information Science from Masdar Institute, UAE, which was created in collaboration with MIT. He received the Ph.D. degree in Interdisciplinary Engineering from Masdar Institute in 2019. From 2019-2020 he was with the Research Institute for Mathematical Sciences (RIMS), Kyoto, Japan as a post-doctoral researcher. Currently, he is a post-doctoral fellow with Khalifa University, UAE. His research interests are centered primarily on the design and analysis of algorithms, mathematical programming, computational theory and their practical applications in Cyber-physical systems and Artificial Intelligence.
\end{IEEEbiography}

\vspace*{-10mm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/ckchau.jpg}}]{Sid Chi-Kin Chau}
is with the Research School of Computer Science at the Australian National University. He was an Associate Professor with the Department of Computer Science at Masdar Institute, which was created in collaboration with MIT, and is a part of Khalifa University. 
His research interests are related to the computing systems and applications for sustainable smart cities by applying Internet-of-things, computational intelligence, advanced algorithms and big data analytics to develop sustainable solutions for smart cities (including smart grid, smart buildings, intelligent vehicles and transportation). He also researches in broad areas of blockchain, Internet-of-things, and algorithms.
Previously, he was a visiting professor with MIT, a senior research fellow with A*STAR in Singapore, a Croucher Foundation research fellow with University College London with a research fellowship awarded by the Croucher Foundation Hong Kong, a visiting researcher with IBM Watson Research Center and BBN Technologies, and a post-doctoral research associate with University of Cambridge. He received the Ph.D. from University of Cambridge with a scholarship by the Croucher Foundation Hong Kong, and B.Eng. (First-class Honours) from the Chinese University of Hong Kong. He is a TPC co-chair of ACM e-Energy 2018, and guest editor for IEEE Journal on Selected Areas in Communications Special Issue on Design and Analysis of Communication Interfaces for Industry 4.0, IEEE Journal of Internet-of- Things Special Issue on Internet-of-Things for Smart Energy Systems, and IEEE Transactions on Sustainable Computing Special Issue on Intersection of Computing and Communication Technologies with Energy Systems. He is an associate editor of IET Smart Grid. He was a co-founder of a start-up specializing in intelligent systems and big data analytics for smart building management.
\end{IEEEbiography}

\vspace*{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,clip,keepaspectratio]{images/khaled.jpg}}]%
{Khaled Elbassioni} received B.S. and M.S. degrees in Computer Science from Alexandria University, Egypt, and a Ph.D. degree in Computer Science from Rutgers University, USA. From 2006 to 2012, he was a senior researcher at Max-Planck Institute for Informatics, Saarbruecken, Germany. He is currently a professor in the Electrical Engineering and Computer Science department at Khalifa University of Science and Technology. His main research interests are in the design and analysis of efficient algorithms, with focus on discrete and continuous optimization, approximation algorithms, game theory and their applications in smart grid and power systems.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/tseng.png}}]%
{Chien-Ming Tseng} received the Ph.D. degree in Interdisciplinary Engineering from Masdar Institute, UAE, in collaboration with MIT in 2017. Currently, he is a Senior Roboticist at Ubiquiti Inc., Taiwan.
\end{IEEEbiography}




